DILBERT: Customized Pre-Training for Domain Adaptation withCategory Shift, with an Application to Aspect Extraction

The rise of pre-trained language models has yielded substantial progress in the vast majority of Natural Language Processing (NLP) tasks. However, a generic approach towards the pre-training procedure can naturally be sub-optimal in some cases. Particularly, fine-tuning a pre-trained language model on a source domain and then applying it to a different target domain, results in a sharp performance decline of the eventual classifier for many source-target domain pairs. Moreover, in some NLP tasks, the output categories substantially differ between domains, making adaptation even more challenging. This, for example, happens in the task of aspect extraction, where the aspects of interest of reviews of, e.g., restaurants or electronic devices may be very different. This paper presents a new fine-tuning scheme for BERT, which aims to address the above challenges. We name this scheme DILBERT: Domain Invariant Learning with BERT, and customize it for aspect extraction in the unsupervised domain adaptation setting. DILBERT harnesses the categorical information of both the source and the target domains to guide the pre-training process towards a more domain and category invariant representation, thus closing the gap between the domains. We show that DILBERT yields substantial improvements over state-of-the-art baselines while using a fraction of the unlabeled data, particularly in more challenging domain adaptation setups.

==> filler.tex <==

Aspect extraction is an important subtask within Aspect Based Sentiment Analysis (ABSA), which aims to extract one or more aspect terms from some text.  As a central task, aspect extraction has received a considerable amount of attention in the literature. 
% indomain ae
 \cite{qiu-etal-2011-opinion} (mine) proposed extracted opinion words and targets using known and extracted opinion words and targets.
through the identification of syntactic relations. The identification of the relations is
the key to the extractions. 

\cite{liu-etal-2015-fine} (mine) used Recurrent Neural Networks (RNN) together with other linguistic features to outperform the older methods of feature rich Conditional Random Fields (CRF) models.

\cite{article} (mine) presented the first deep learning approach to aspect extraction. They used seven layer deep convolutional neural network together with other linguistic patterns.

\cite{wang-etal-2016-recursive,10.5555/3104482.3104602} (from other paper) integrated recursive neural networks and conditional random
fields into a unified framework for explicit aspect and opinion terms co-extraction. Their model propagates information between aspect and opinion terms in sort of multi-task learning.





% cross domain aspect extraction

Due to the difficulties in fine-grained adaptation, there exist very few methods for cross-domain aspect extraction.
\cite{10.5555/3298023.3298068} (mine) combined rule-based, unsupervised opinion target extraction with neural network based supervised models to achieve
better performance in a cross-domain setting. They collected auxiliary labels for both domains using rules that use syntactic patterns to detect potential opinion
targets. After collecting the auxiliary labels they trained different networks on both the true source labels and on the auxiliary labels from both domains. 
Nevertheless, their performance is highly dependent on the quality of the manually defined rules and the knowledge of a sentiment lexicon.

\cite{wang-pan-2018-recursive} (from other paper) applied recursive neural networks with pre-generated dependency trees to build dependency-sensitive representation for each word, in which correspondences across domains are built according to syntactic structure. This approach requires a dependency parser that is not guaranteed to be accurate, especially on user-generated texts, which may lead to poor extraction performance.

\cite{li-etal-2019-transferable} (from other paper) proposed a selective adversarial learning strategy to learn domain-invariant representations of aspect words. However, they still use classic base models such as LSTM and don't incorporate the power of pre-trained text encoders such as BERT.

\cite{liang2020weakly}, not really comparable to our work, they use category labels on both the source and target domains to improve aspect extraction.

Recently, \cite{gong-etal-2020-unified} (mine) were the first to use pre-trained text encoders such as BERT. However, in their work they mostly show how you can use your source and target data in better ways but don't show how you can use large amounts of unlabled data for better pre-training in advance. Moreover they use BERT as a baseline and don't really adapt its learning for the domain adaptation case.


\subsection{Domain Adaptation}
 DA is a common challenge for machine learning and in particular for NLP. DA has a variety of setups, but this work is mainly on unsupervised DA. In this setup, unlabeled data is available from both the source domain and the target domain, but labeled data is only available in the source domain. 
 
 
There are different approaches to DA, some of them are: instance reweighting \cite{NIPS2008_3550}, sub-sampling from both domains \cite{10.5555/3104482.3104602} and learning a common representation for both domains (DReL). This is the approach we decided to take here.
\subsection{Unsupervised Domain Adaptation with DReL}
DRel typically consists of two major steps: representation learning and classification. In the first step, a representation model is trained on the unlabeled data from the source and target domains. In the second step, training a supervised model on the source domain labeled data. Ultimately, every example that is provided to the task specific model is first represented by the representation model. This is true both during the training phase and during the test phase when the model is applied to the target domain.  

Unsupervised DA through representation learning has followed two main avenues. The first avenue consists of works that aim to explicitly build
a feature representation that bridges the gap between the domains. A seminal framework in this
line is structural correspondence learning (SCL,
\citet{blitzer-etal-2007-biographies, ziser-reichart-2017-neural,ziser-reichart-2018-pivot}), that splits the feature space into pivot and non-pivot features. A
large number of works have followed this idea and we discuss it below.
Works in the second avenue learn cross-domain
representations by training autoencoders (AEs) on
the unlabeled data from the source and target domains. This way they hope to get a more robust
representation, which is hopefully better suited for
DA. \citet{ziser-reichart-2017-neural,ziser-reichart-2018-pivot} married these approaches and presented pivot-based approaches where the representation model is based on DNN encoders.

\subsection{Pivot-based Domain Adaptation}
Proposed by \citet{blitzer2006domain,blitzer-etal-2007-biographies} through their SCL
framework, the main idea of pivot-based DA is to
divide the shared feature space of the source and
the target domains to two complementary subsets:
one of pivots and one of non-pivots. Pivot features
are defined based on two criteria: (a) They are frequent in the unlabeled data of both domains; and
(b) They are prominent for the classification task
defined by the source domain labeled data. Nonpivot features are those features that do not meet
at least one of the above criteria. 
\citet{ziser-reichart-2018-pivot} have presented the
Pivot Based Language Model (PBLM), which incorporates pre-training and pivot-based learning.
PBLM is a variant of an LSTM-based language
model, but instead of predicting at each point the
most likely next input word, it predicts the next input unigram or bigram if one of these is a pivot (if
both are, it predicts the bigram), and NONE otherwise. In the unsupervised DA pipeline PBLM
is trained on the source and target unlabeled data.
Then, when the task classifier is trained and applied to the target domain, PBLM is employed as a contextualized word embedding layer.
Recently, \cite{ben-david-etal-2020-perl} presented PERL, which employs pivot features in order to learn a representation that bridges the gap between two
domains. Contrary to previous pivot-based DA
representation models, it exploits unlabeled data
from the source and target domains, and also from
massive out of source and target domain corpora.
It refines some of the pre-trained encoder weights, based on a pivot-based objective that is optimized on unlabeled data from the source and target domains.

\subsection{Contextualized Word Embedding Models}
Contextualized word embedding (CWE) models
are trained on massive corpora \citet{peters-etal-2018-deep}.  Contributions of such models to state-of-the-art solutions to NLP tasks are already well-known.
CWE models typically follow three steps: (1)
Pre-training: Where a DNN (referred to as the encoder of the model) is first trained on massive un-
labeled corpora which represent a broad domain
(such as English Wikipedia); (2) Fine-tuning: An
optional step, where the encoder is refined on
unlabeled text of interest; and (3) Supervised task
training: Where task specific layers are trained on
labeled data for a downstream task of interest.
DILBERT employs a pre-trained encoder, BERT
in this paper. BERT’s architecture is based on
multi-head attention layers, trained with a two component objective: (a) MLM and (b) Is-nextsentence prediction (NSP). 
MLM is a modified language modeling objective, adjusted to self-attention models. When
building the pre-training task, all input tokens have
the same probability to be masked. After the
masking process, the model has to predict a distribution over the vocabulary for each masked token given the non-masked tokens. The input text
may have more than one masked token, and when
predicting one masked token information from the
other masked tokens is not utilized. 
DILBERT changes effect mainly the second step while modifying the MLM task to a more suitable task for the setup of Domain Adaptation.

==> misc.tex <==
\section{misc}
Use \cite{xu-etal-2018-double} (mine) has shown that incorporating domain word embeddings greatly improved the performance of Aspect Extraction. to justify traning in domain word embeddings.
From  Aspect Term Extraction for Sentiment Analysis: New Datasets, New Evaluation Measures and an Improved Unsupervised Method (https://www.aclweb.org/anthology/W14-1306.pdf)

The most commonly used dataset is that of Hu and Liu (2004), which contains reviews of only five particular electronic products (e.g., Nikon Coolpix 4300). Each sentence is annotated with aspect terms, but inter-annotator agreement has not been reported.1 All the sentences appear to have been selected to express clear positive or negative opinions. There are no sentences expressing conflicting opinions about aspect terms (e.g., “The screen is clear but small”), nor are there any sentences that do not express opinions about their aspect terms (e.g., “It has a 4.8-inch screen”). Hence, the dataset is not entirely representative of product reviews.



\section{Domain Adaptation with DILBERT}
Domain Invariant Learning with Bert 
\section{Experimental Setup}
Talk about services and devices.

Talk about hotels.

Talk about evaluation - em.


\section{Results}
Talk about sentiment pivots.
\section{Ablation Analysis}
\section{Conclusions}



